Benchmarks for Reinforcement Learning with Biased Offline Data and Imperfect Simulators

In many reinforcement learning (RL) applications one cannot easily let the agent act in the world; this is true for autonomous vehicles, healthcare applications, and even some recommender systems, to name a few examples. Offline RL provides a way to train agents without real-world exploration, but is often faced with biases due to data distribution shifts, limited coverage, and incomplete representation of the environment. To address these issues, practical applications have tried to combine simulators with grounded offline data, using so-called hybrid methods. However, constructing a reliable simulator is in itself often challenging due to intricate system complexities as well as missing or incomplete information. In this work, we outline four principal challenges for combining offline data with imperfect simulators in RL: simulator modeling error, partial observability, state and action discrepancies, and hidden confounding. To help drive the RL community to pursue these problems, we construct ``Benchmarks for Mechanistic Offline Reinforcement Learning'' (B4MRL), which provide dataset-simulator benchmarks for the aforementioned challenges. Our results suggest the key necessity of such benchmarks for future research.

==> figures/results_table.tex <==






    

% \begin{table}[t]
%   \caption{Results on MuJoCo HalfCheetah task. All results shown in this table are normalized as suggested in D4RL. Columns represent different RL approaches and algorithms, while rows represent different type of dataset. The top part of the table corresponds to D4RL datasets, and the bottom part corresponds to datasets created specifically for the partial-observability challenges described in \Cref{subsec:benchmarks}. The \emph{last-observation} row represents a dataset generated by an agent that does not observe the last dimension of the HalfCheetah full state, and trains only on the last observation. The \emph{3-obs history} row represents a dataset generated similarly, but the agent trains on a history of the last 3 observations.}
%   \label{tab:halfcheetah}
%   \centering
%   \begin{tabular}{c|c|cc|cc|cc}
%     \toprule
%     & & \multicolumn{2}{c}{Online-RL (sim)} & \multicolumn{2}{c}{Offline-RL (data)} & \multicolumn{2}{c}{Hybrid-RL}    \\
%     \cmidrule{3-8}
%     Dataset     &  Discrepancy  & TD3 & SAC & MOPO & TD3-BC & H2O & \ours \\
%     % ---------------------------------------------------------------------------------------------------------------
%     % ---------------------------------------------------------------------------------------------------------------
%     % ---------------------------------------------------------------------------------------------------------------
%     \midrule
%     \multicolumn{8}{c}{D4RL datasets -- transition error} \\
%     \midrule
%     \multirow{2}{*}{Random}
%     & Friction  & 45.0 $\pm$ 9.5 & 65.9 $\pm$ 11.7 & \multirow{2}{*}{36.2 $\pm$ 0.9} & \multirow{2}{*}{12.2 $\pm$ 0.5} & 30.4 $\pm$ 12.2 & 40.0 $\pm$ 2.0 \\
%     & Gravity   & 35.3 $\pm$ 1.9 & 35.1 $\pm$ 2.4 &  &  & 36.7 $\pm$ 2.4 & 36.1 $\pm$ 2.5 \\
%     \midrule
%     \multirow{2}{*}{Medium}
%     & Friction  & 45.0 $\pm$ 9.5 & 65.9 $\pm$ 11.7 & \multirow{2}{*}{66.1 $\pm$ 0.3} & \multirow{2}{*}{48.3 $\pm$ 0.1} & 55.7 $\pm$ 5.9 & 73.9 $\pm$ 0.4 \\
%     & Gravity   & 35.3 $\pm$ 1.9 & 35.1 $\pm$ 2.4 &  &  & 51.0 $\pm$ 10.4 & 72.9 $\pm$ 0.8 \\
%     \midrule
%     \multirow{2}{*}{Medium replay}
%     & Friction  & 45.0 $\pm$ 9.5 & 65.9 $\pm$ 11.7 & \multirow{2}{*}{67.8 $\pm$ 2.4} & \multirow{2}{*}{42.8 $\pm$ 2.9} & 49.8 $\pm$ 3.6 & 68.6 $\pm$ 1.4 \\
%     & Gravity   & 35.3 $\pm$ 1.9 & 35.1 $\pm$ 2.4 &  &  & 54.8 $\pm$ 3.3 & 66.5 $\pm$ 0.6 \\
%     \midrule
%     \multirow{2}{*}{Medium expert}
%     & Friction  & 45.0 $\pm$ 9.5 & 65.9 $\pm$ 11.7 & \multirow{2}{*}{49.2 $\pm$ 14.5} & \multirow{2}{*}{84.3 $\pm$ 5.2} & 18.9 $\pm$ 1.8 & 99.2 $\pm$ 5.1 \\
%     & Gravity   & 35.3 $\pm$ 1.9 & 35.1 $\pm$ 2.4 &  &  & 41.2 $\pm$ 2.9 & 95.1 $\pm$ 2.0 \\
%     % ---------------------------------------------------------------------------------------------------------------
%     % ---------------------------------------------------------------------------------------------------------------
%     % ---------------------------------------------------------------------------------------------------------------
%     \midrule
%     \multicolumn{8}{c}{D4RL datasets -- observation / action error} \\
%     \midrule
%     \multirow{3}{*}{Random}
%     & Obs noise  &  &  &  & \multirow{3}{*}{12.2 $\pm$ 0.5} &  &  \\
%     & Partial obs low  &  83.3 $\pm$ 3.3 &  &  &  &  &  \\
%     & Partial obs high  &  &  &  &  &  &  \\
%     & Action noise   &  &  &  &  &  &  \\
%     \midrule
%     \multirow{3}{*}{Medium}
%     & Obs noise  &  &  &  & \multirow{3}{*}{48.3 $\pm$ 0.1} &  &  \\
%     & Partial obs low  &  83.3 $\pm$ 3.3 &  &  &  & 54.4 $\pm$ 5.5 &  76.1 $\pm$ 2.0\\
%     & Partial obs high  &  &  &  &  &  &  \\
%     & Action noise   &  &  &  &  &  &  \\
%     \midrule
%     \multirow{3}{*}{Medium replay}
%     & Obs noise  &  &  &  & \multirow{3}{*}{42.8 $\pm$ 2.9} &  &  \\
%     & Partial obs low  & 83.3 $\pm$ 3.3 &  &  & & 54.7 $\pm$ 1.2 & 66.0 $\pm$ 3.8 \\
%     & Partial obs high  &  &  &  &  &  &  \\
%     & Action noise   &  &  &  &  &  &  \\
%     \midrule
%     \multirow{3}{*}{Medium expert}
%     & Obs noise  &  &  &  & \multirow{3}{*}{84.3 $\pm$ 5.2} &  &  \\
%     & Partial obs low  & 83.3 $\pm$ 3.3 &  &  &  & 43.4 $\pm$ 3.8 & 101.6 $\pm$ 1.0 \\
%     & Partial obs high  &  &  &  &  &  & 79.9 $\pm$ 7.0 \\
%     & Action noise   &  &  &  &  &  & 29.0 $\pm$ 10.4 \\
%     % ---------------------------------------------------------------------------------------------------------------
%     % ----------------------------- D4RL - confounding errors - hidden-dims observations ----------------------------
%     % ---------------------------------------------------------------------------------------------------------------
%     \midrule
%     \multicolumn{8}{c}{D4RL datasets -- confounding error with hidden observations} \\
%     \midrule
%     Random & Gravity  &  &  &  &  &  &  \\
%     \midrule
%     Medium & Gravity  &  &  &  &  &  &  \\
%     \midrule
%     Medium replay & Gravity  &  &  &  &  &  &  \\
%     \midrule
%     Medium expert & Gravity  &  &  &  &  &  &  \\

%     % ---------------------------------------------------------------------------------------------------------------
%     % ---------------------------------------------------------------------------------------------------------------
%     % ---------------------------------------------------------------------------------------------------------------
%     \midrule
%     \multicolumn{8}{c}{Datasets with partially observed states} \\
%     \midrule
%     % \multirow{2}{*}{Medium} 
%     Last-observation
%     & Gravity   & 35.3 $\pm$ 1.9 & 35.1 $\pm$ 2.4 & 55.1 $\pm$ 0.4 & 45.9 $\pm$ 0.1 & 45.8 $\pm$ 5.1 & 69.8 $\pm$ 3.2     \\
%     \midrule
%     % \multirow{2}{*}{3-obs history}
%     3-obs history
    
%     & Gravity   & 35.3 $\pm$ 1.9 & 35.1 $\pm$ 2.4 & 56.5 $\pm$ 0.8 & 51.7 $\pm$ 0.3 & 52.5 $\pm$ 0.8 & 68.3 $\pm$ 1.9     \\
%     \bottomrule
%   \end{tabular}
% \end{table}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> mech_discrepencies.tex <==
While simulators allow us to extrapolate outside our data manifold \uri{this requires explanation, should go slower - unless it will appear in the previous section}, their errors and biases can easily propagate and cause poor  agent performance. On the other hand, offline data avoids the inherent biases of simulators, yet is limited by finite data, partial observability and hidden confounders, which in turn may also bring about unbounded bias \uri{cite}. To overcome these challenges, we propose to combine simulation and data \uri{shouldn't this say something like ``researchers have recently turned to approaches combining simulation and data'', with citations?}, while taking careful account of their discrepancies and tradeoffs, and present several axes along which simulators might fall short in terms of modelling the true task. 

We focus on four challenges. \uri{add numbers, and each should have a clear name} Particularly, we discuss the biased transition and observation functions of dynamical simulators. This bias propagates in time, aggregating errors over long horizons. Then, we describe how partial observability in the offline data can affect our ability to solve a problem. We show how the data generating agent's ability to view latent states can drastically affect performance, or even our ability to use the data. We then discuss possible discrepancies between the offline data and the simulation environment, bringing about further challenges in combining them. These include discrepancies in state representations, action space definitions, and various unknown delays in action execution. \guy{are we still doing delays?}

\uri{not sure this last paragraph is needed - possible better to just give the four, with mathematical definitions and all} 

\paragraph{1. Simulator Model Bias.}

The first (and perhaps simplest) discrepancy between simulator and data is the bias in the simulator itself. While data is mostly assumed to be unbiased (i.e., sampled from the true model distribution)\uri{this directly contradicts something we say earlier, we know data can be biased, that the whole point of merging the two approaches...} \guy{I think there's a difference between saying that learning from offline data can cause biases in your decisions vs saying the data itself is biased. We're assuming the data itself is coming from the true distribution, so it is not biased w.r.t. that distribution.}, models are often biased and wrong. Figure \guy{ref figure} depicts possible modeling errors in simulators. To this end, we assume our simulator is a Partially Observable Markov Decision Process (POMDP), into which errors can be injected at one of the following: initial state distribution, transition model, observation model, or reward model. Error here means a some systemic difference between the simulator POMDP and the true POMDP of the environment. Later in this section we also discuss bias induced by misspecification of the state and action sets themselves.  \uri{add example}

\paragraph{2. Partial Observability in Simulators.}

Another discrepancy that often occurs is in our ability to simulate only parts of the observation space. To that end, we are often relying on simulators that are capable of abstracting particular aspects of the problem, or sometimes explicitly model only specific elements. As a simplification of this setting we may consider simulators which simply do not model part of the observation space. They may be biased w.r.t. their transition, and do not include certain information. For example, an autonomous driving simulator may simulate the physics and movement of vehicles and pedestrians, yet not model particular facial expressions of the humans involved. While such a simulator is still useful for solving the task at hand, further and higher resolution information in the data can greatly improve overall performance. \uri{ need to clarify why isn't this just a special case of \textbf{1.} above}

\paragraph{3. Hidden Confounders in Data.} 

The presence of confounding variables poses a significant challenge when utilizing observational data for decision-making. Confounding occurs when in the process that generated the offline data, unobserved factors exerted influence on both the outcome and the decisions made by the agent. This can lead to unbounded bias, a result which is well known from the causal inference literature \uri{cite}. This issue becomes particularly pertinent in sequential decision-making scenarios and can substantially impact the performance of learned policies. Hidden confounding is prevalent in diverse real-world applications, including autonomous driving, where unobserved factors like road conditions affect the behavior of the observed policy, and healthcare, where for example unrecorded patient information or patient preferences may influence the decisions made by physicians.

Effectively addressing confounding in offline RL is paramount to ensure the reliability and effectiveness of learned policies. Research has attempted to develop methodologies to account for confounding bias, including: the identification of hidden confounders \guy{cite}, using interventions or additional data sources \guy{cite}, and the quantification and integration of uncertainty arising from confounding into the learning process \guy{cite}. There is a crucial need for benchmarks and datasets specifically designed to address this issue, enabling researchers to compare and evaluate different methods for handling confounding bias in offline reinforcement learning.

\uri{ same here, need to clarify why isn't this just a special case of \textbf{1.} above}

\paragraph{4. State and Action Discrepancies.}

One of the substantial challenges in merging simulation and offline data lies in inconsistencies between state and action definitions in simulation environments and offline data. Every action taken by an agent in the real environment and every state it visits can be nuanced and multifaceted. Simulators, on the other hand, have to abstract these complexities into a more manageable and computationally feasible representation. As a result, there can be a disconnect in how states and actions are represented in these two different systems.

State and action representation can vary significantly depending on the system used. In simulators, these might be represented with a specific level of detail or abstraction depending on the complexity of the environment and the computational resources available. For example, an autonomous driving system, the state can be represented as the positions and velocities of nearby cars. However, in real-world data, the state might also include factors such as the condition of the road, the weather, and the behavior of other drivers. In a flight simulator, the action of changing altitude might be simplified to increase or decrease, while in real-world flight data, the action might include intricate details like the rate of ascent or descent, angle of attack, and airspeed. 

Furthermore, real-world time delays in action execution might not be mirrored in simulators, adding another layer of complexity. For instance, in a real-world driving scenario, there is a brief delay between when a driver decides to apply the brakes and when the car actually begins to slow down due to the physical process involved. However, a simulator might implement the braking action instantaneously, which can cause discrepancies when combining simulation and offline data.



==> related.tex <==
%The applicability of online-RL methods in various real-world domains is restricted due to their dependence on environment interaction for training.
%Such interactions may not be feasible in many domains such as healthcare \citep{gottesman2018evaluating}, \ori{add fields and citations.}.
%This limitation has been addressed by two main paradigms: training on a simulator, and training on offline data. 

% Online - sim2real gap
Simulation based RL has long been recognized as a challenging task, due to the dynamics gap between the simulation and the real world dynamics.
This problem, commonly referred as sim2real gap, has fueled extensive research throughout the years \citep{kadian2020sim2real}. \ori{expand this}

In many applications, creating a reliable simulator is impractical due to missing some of the modelling knowledge, requiring access to unmeasured variables, or holds a dynamics gap that makes training infeasbile.
This issue has led to recent advances in finding offline methods to optimize policies by avoiding vising regions not covered in the dataset either through pessimism, or by computing the models' uncertainty \citep{levine2020offline,fujimoto2019off,kumar2019stabilizing,nachum2019algaedice,yu2020mopo, kidambi2020morel,kumar2020conservative, jin2021pessimism,kostrikov2021offline}.
These methods, however, do not take into account the possible inherent problem of hidden confounders in the data.
Hidden confounders may cause bias in the dataset that cannot be reduced even if more data is accessible, as this problem cannot be modeled as a partially-observable environment.

This work aims to incentivize research in finding hybrid-RL methods that leverages both offline biased data and imperfect simluators, hoping to improve learning efficiency, stability, and generalization capabilities.
Such methods have started to arise recently \cite{song2022hybrid,niu2022trust,niu2023re}, but without a standardized method to benchmark and compare.
The most common benchmark for offline-RL methods is D4RL \citep{fu2020d4rl}.
This work provides different levels of datasets, categorized mainly by the score achieved by the underlying data-generating-agent, from completely random actions to expert.
Although these benchmarks cover important aspects and challenges in offline-RL, like limited data coverage, they do not provide a benchmark that addresses hidden confounders in the data.
Several benchmarks for offline-RL methods have been developed over recent years \citep{fu2020d4rl,fujimoto2019off,qin2022neorl,wu2019behavior,gulcehre2020rl}.
However, they do not directly address hidden confounders in the dataset and do not offer a standardized method for benchmarking hybrid-RL methods.

